Few-Shot Conversational Dense Retrieval

Dense retrieval (DR) has the potential to resolve the query understanding challenge in conversational search by matching in the learned embedding space. However, this adaptation is challenging due to DR models' extra needs for supervision signals and the long-tail nature of conversational search. In this paper, we present a Conversational Dense Retrieval system, ConvDR, that learns contextualized embeddings for multi-turn conversational queries and retrieves documents solely using embedding dot products. In addition, we grant ConvDR few-shot ability using a teacher-student framework, where we employ an ad hoc dense retriever as the teacher, inherit its document encodings, and learn a student query encoder to mimic the teacher embeddings on oracle reformulated queries. Our experiments on TREC CAsT and OR-QuAC demonstrate ConvDR's effectiveness in both few-shot and fully-supervised settings. It outperforms previous systems that operate in the sparse word space, matches the retrieval accuracy of oracle query reformulations, and is also more efficient thanks to its simplicity. Our analyses reveal that the advantages of ConvDR come from its ability to capture informative context while ignoring the unrelated context in previous conversation rounds. This makes ConvDR more effective as conversations evolve while previous systems may get confused by the increased noise from previous turns. Our code is publicly available at https://github.com/thunlp/ConvDR.

==> Arxiv/00_abs.tex <==
\begin{abstract}
Conversational retrieval has recently been developed to satisfy information seeking in multi-round interactions between humans and intelligent agents. Existing systems usually employ sparse retrievers, such as BM25, to search documents. In general conversations, user utterances are usually context-dependent and under-specified, which encourages existing work focus on explicitly rewriting de-contextualized questions for sparse retrievers. However, the explicitly reformulating or expanding questions always includes uninformative and confusing contents, misleading conversational retrieval models. In this paper, we propose a conversational dense retriever, ConvANCE, that directly encodes current question and its historical utterances as a dense representation and conducts text retrieval in an embedding space, overcoming the vocabulary mismatch problem of sparse retrievers. To broaden the advantage of ad hoc dense retrievers, we employ the state-of-the-art ad hoc dense retriever ANCE to conduct a well-trained embedding space of documents and map question representations into this document embedding space. Our experiments demonstrate the effectiveness of ConvANCE by achieving 11.6\% and 37.8\% improvements on TREC CAsT 2019 and OR-QuAC compared to previous state-of-the-art query rewriter and showing even better performance than manually reformulated questions, while training with few data. Our code will be open-sourced.
\end{abstract}

==> Arxiv/01_intro.tex <==
\section{Introduction}
With the rapid development of intelligent assistant systems such as Alexa, Siri and Cortana, the information acquisition goal of Information Retrieval (IR) gradually moves to satisfy conversational experiences, which is viewed as a next generation IR direction~\cite{yu2020few}.

\input{Figures/fig-model}
Conversational retrieval aims at retrieving relevant documents for a series of questions ("utterances") issued by a user in a multi-round conversation.
Under multi-round interactions in a conversation, the utterances are usually coherent in the topic, may contain references to previous discussions and ignore some mentioned concepts. Figure~\ref{fig:model} shows a short example from TREC Conversational Assistance Track (CAsT) 2019. The user starts with a general question regarding the Bronze Age collapse ($Q_1$), and then explicitly or implicitly references it in $Q_2$ and $Q_3$. Compared to the de-contextualized manually rewritten questions (denoted with *), such context-dependent, under-specified and implicit questions raise more challenges for retrieval systems~\cite{dalton2020cast,qu2020orqa}. 

Thus, modeling conversation history becomes the key challenge of conversational retrieval. Recent work mainly employs a \textit{rewrite-retrieve} pipeline, i.e.  explicitly rewriting the contextualized questions into de-contextualized ones and then feeding the rewritten questions into an ad hoc retrieval system. Various methods have been proposed to \textit{rewrite} conversational questions. Some of them~\cite{yang2019query,kumar2020making,voskarides2020query} picks up necessary and informative tokens from historical utterances by either heuristic or neural methods to expand current questions, making the question more informative. Question reformulation~\cite{yu2020few,cast2019overview,elgohary2019canard,lin2020query,vakulenko2020question} leverages neural models to capture necessary information from current and its historical utterances to generate de-contextualized questions. After explicit question rewriting, existing conversational retrieval systems mainly employ sparse retrieval methods (e.g. BM25) to retrieve documents based on discrete bag-of-words matching, which is consistent with conventional ad hoc retrieval paradigms. 

The \textit{rewrite-retrieve} pipeline has shown promising results~\cite{cast2019overview}, but it often requires using complicated techniques, such as combining expanded tokens from different sources~\cite{kumar2020making} or fusing multiple runs~\cite{lin2020query}, to get comparable results to directly applying manually rewritten questions. The weakness of those \textit{rewrite-retrieve} methods roots from a) the vocabulary mismatch problem intrinsic to sparse retrievers; b) the drift of user intent after inaccurate question rewriting~\cite{vakulenko2020question,lin2020query}. Recently, dense retrievers (DRs)~\cite{xiong2020approximate,xiong2020dense,karpukhin2020dense} alleviate the vocabulary mismatch problem by employing the pretrained language model BERT~\cite{devlin2019bert} to separately encode both queries and documents as dense representations and conducting semantic retrieval in an embedding space. Qu et al.~\cite{qu2020orqa} further extend DR into conversational setting by concatenating current utterance with its history questions and training with a large amount of annotated data. Research has shown that DRs thrive from end-to-end training and require large scale training data to learn good text representations~\cite{xiong2020approximate}. However, conversational retrieval tasks are usually few-shot, i.e. have limited annotated relevance labels for training~\cite{dalton2020cast,qu2020orqa}, even in many large enterprises. To this end, we see DRs as single-turn conversational retrievers and propose to grab ranking knowledge from vanilla single-turn DRs to build conversational DRs.

In this paper, we come up with a simple yet effective conversational retrieval model, Conversational ANCE (\convance{}), based on the state-of-the-art ad hoc dense retrieval model ANCE~\cite{xiong2020approximate}.
Figure~\ref{fig:model} presents the motivation of \convance{}. \convance{} aims to learn customized representations of current questions and map them into the well-trained embedding space of ANCE for text retrieval. We first get the representation for the current question by using \convance{} to encode current and historical utterances in a conversation. Then we regard \convance{} as a ``student'' model and optimize the conversational question representation of \convance{} to be asymptotic with respect to the manual question representation of the ``teacher'' model ANCE.
Different from question rewrites, \convance{} encodes all information from the historical utterances, is optimized to learn informative question representations and broadens the advance of well-trained ad hoc retrievers to conversational retrievers.

Experiments on two conversational retrieval datasets, CAsT-19~\cite{dalton2020cast} and QR-QuAC~\cite{qu2020orqa}, demonstrate the effectiveness of \convance{} by outperforming the previous state-of-the-art question rewriter based models~\cite{yu2020few} with 11.6\% and 37.8\% improvements and achieving even better performance than the manually reformulated questions. Our analyses show that \convance{} has the ability to pick up more informative utterances from previous turns, better comprehends complex conversational questions and avoids additional errors and misleading from reformulated questions. These advances help \convance{} conduct more tailored question representations for conversational retrieval. Moreover, \convance{} provides a simple but effective training paradigm to map the representations of conversational questions into a well-trained embedding space of ad hoc retriever, thriving on the few-shot conversational retrieval.


%In the rest of this paper, Section 2 discusses related work and Section 3 presents \convance{}. Experiment settings and evaluation results are discussed in Section 4 and Section 5. We conclude in Section 6.

==> Arxiv/02_related.tex <==
\section{Related Work}


Information Retrieval (IR) aims to find relevance documents to satisfy information needs of users. Many language models usually employ text retrievers to seek information from a large-scale document collection, such as open domain question answering~\cite{chen2017reading} and fact verification~\cite{thorne2018fact}.
Conversational retrieval~\cite{radlinski2017theoretical,trippas2018informing} comes up with a new IR problem and focuses on conversational information seeking with multi-round interactions, serving for conversational question answering~\cite{choi2020quac,reddy2019coqa}.

The recently released datasets, TREC Conversational Assistance Track (CAsT)~\cite{dalton2020cast} and OR-QuAC~\cite{qu2020orqa}, thrive on the development of conversational retrieval systems. Different from general IR systems, the questions in conversations usually omit some necessary concepts, causing they are context-dependency and under-specified. Thus, existing work formulates the task of information seeking by clarifying the conversational questions in open-domain conversational systems and conducting context-independent questions to adapt to general IR models~\cite{aliannejadi2019asking}.

One direct solution is using coreference resolution to clarify the questions. However, the coreference in conversation differs from the typical coreference in other text genres~\cite{cast2019overview}, which leads off-the-shelf coreference models show less effectiveness on resoluting coreference in conversations and harms the retrieval performance~\cite{cast2019overview}. Some work also attempts to reformulate conversational questions~\cite{lin2020query} into de-contextualized ones or expand questions~\cite{yang2019query}. They aim to include necessary information from the conversation history for retrieval. One of the top performing systems in TREC CAsT is ATeam’s conversational query rewriter~\cite{cast2019overview}, which feeds the previous and current questions in the session into the pretrained language model GPT-2~\cite{radford2019language} and generates de-contextualized questions. Yu et al.~\cite{yu2020few} further fine-tune GPT-2 using large amounts of ad hoc search sessions through rules and self-supervised learning to significantly improve the rewriter's performance. Kumar et al.~\cite{kumar2020making} further combine multi-view query representations provided by question expansion and question reformulation for reranking.

Most previous pipeline models use a TF-IDF/BM25 retriever as the first step retrieval in conversational retrieval systems~\cite{cast2019overview,kumar2020making} and is compelled to conduct additional question expansion and reformulation. Nevertheless, the sparse retriever has vocabulary mismatch problem and becomes the bottleneck of the retrieval system~\cite{xiong2020approximate}. Qu et al.~\cite{qu2020orqa} further leverage dense retriever~\cite{karpukhin2020dense} to encode current questions and its history utterances as the dense representation and avoid incorporating additional misunderstandings from explicitly rewritten questions. Dense retrieval usually leverages BERT~\cite{devlin2019bert} to encode questions and documents and conducts efficient retrieval in an embedding space with the support of approximate nearest neighbor (ANN)~\cite{johnson2019billion} search. Existing work in dense retrieval focuses on training BERT with contrastive examples~\cite{xiong2020dense, xiong2020approximate,karpukhin2020dense}. ANCE~\cite{xiong2020approximate} achieves the state-of-the-art performance in ad hoc retrieval and conducts effective sampling strategies to avoid diminishing gradient norms for a stable and robust training process~\cite{xiong2020approximate}. However, different from ad hoc retrieval, the conversational retrieval datasets~\cite{dalton2020cast, qu2020orqa} contain few training data, which may not fully train neural IR models~\cite{zhang2020rapidly,qiao2019understanding} and limits the performance of dense retriever~\cite{xiong2020approximate}.

Knowledge Distillation (KD)~\cite{hinton2015distilling,bucilu2006model,wang2020knowledge} provides an opportunity to alleviate the data scarcity for training neural networks. It aims to transfer knowledge from one well trained network to another network, which can be regarded as the ``teacher-student'' mechanism~\cite{hinton2015distilling,park2019feed,kim2018paraphrasing,chung2020feature}. The knowledge distillation has been widely used to enable human to quickly learn complex concepts and show the effectiveness on guiding the ``student'' network learn. Benefited from teacher-student interactions, the student model can learn complex patterns on few-shot scenarios~\cite{gutstein2008knowledge} or conduct lighter and smaller model with comparable performance~\cite{sanh2019distilbert}. With KD, conversational retrieval system is able to better capture necessary information from conversation history and learn to extract match patterns with few training data.

==> Arxiv/03_method.tex <==
\section{Methodology}\label{model}
In this section, we first recap preliminaries in conversational search. Then we present our Conversational Dense Retrieval (\convance{}) framework and its teacher-student few-shot learning strategy.

% This section describes our Conversational Dense Retrieval (\convance{}) model to satisfy information seeking in multi-turn conversations. We first introduce preliminaries of conversational retrieval (Sec.~\ref{model:preliminary}), then describe the dense retrieval method for conversational retrieval (Sec.~\ref{model:dense}) and finally, presents our \convance{} to alleviate data dependency with a teacher-student learning method for few-shot conversational dense retrieval (Sec.~\ref{model:kd}).

\subsection{Preliminary}\label{model:preliminary}
Conversational retrieval aims to search document $d$ from a document collection $D$ according to the current query $q_k$ and all its history queries $Q_{k-1} = \{q_i\}_{i=1}^{k-1}$ in a conversation.

The conversational queries imply contexts from previous queries $Q_{k-1}$, making these queries are context-dependent, under-specified and hard understanding~\cite{radlinski2017theoretical, trippas2018informing, dalton2020cast}. To resolve the context dependency of conversational queries, recent research aims to retrofit the conversational query $q_k$ into the de-contextualized query ${q_k}'$ through query rewriters~\cite{cast2019overview,yu2020few}:
\begin{equation}
    {q_k}' = \text{Query Rewriter}(Q_{k-1}, q_k),
\end{equation}
which aims to mimic the ad hoc query that includes all information and satisfies users' information need for searching~\cite{cast2019overview}. 

These conversational queries are reformulated in the sparse bag-of-word space and employ the standard sparse retrieval BM25 to search candidate documents from the document collection $D$ and form the candidate document collection $D^*$:
\begin{equation}
     D^* = \text{BM25} ({q_k}', D).
\end{equation}
Then for each document $d$ in the candidate document set $D^*$, we can leverage BERT~\cite{devlin2019bert} to get the token representations $H({q_k}',d)$ for the retrofitted query ${q_k}'$ and document $d$:
\begin{equation}\label{eq:rerank:qr}
     H(q_k,d) = \text{BERT} (\text{[CLS]};{q_k}';\text{[SEP]}; d; \text{[SEP]}), 
\end{equation}
where ; denotes the concatenation operator. [CLS] and [SEP] are special tokens in BERT. The representation $H_0({q_k}',d)$ of the first token [CLS] is regarded as the ranking feature of the pair of ${q_k}'$ and $d$. Then the ranking score $f({q_k}',d)$ can be calculated:
\begin{equation}\label{eq:rerank:mlp}
     f({q_k}',d) = \text{MLP}(H_0({q_k}',d)),
\end{equation}
where MLP is the multi-layer perceptron. Finally, we rerank the candidate document set $D^*$ according to the ranking score $f({q_k}',d)$.

The vocabulary mismatch problem~\cite{croft2010search} lain in sparse retrievers is more severe in the conversational search system and has become the obstacle for conversational retrieval, which derives from retrofitted queries that usually incorporate more errors and still underperform manually reformulated queries.





\subsection{Conversational Dense Retrieval}\label{model:dense}
To overcome the vocabulary mismatch problem, \convance{} leverages dense retriever~\cite{xiong2020dense,xiong2020approximate,karpukhin2020dense} to replace sparse retriever in conversational search. \convance{} first encodes each conversational question, then directly matches documents of the document collection $D$ in the learned embedding space~\cite{qu2020orqa} and finally forms the candidate document collection $D^*$. The key part of \convance{} is learning tailored query representations in the embedding space that satisfy user's information needs according to the historical queries $Q_{k-1}$.


Following Qu et al.~\cite{qu2020orqa}, we directly encode the current query $q_k$ and historical queries $Q_{k-1}$ to avoid incorporating errors from retrofitted query~\cite{yu2020few,cast2019overview}.
Given the current query $q_k$ and a document $d$ from the document collection $D$, we can get all token representations $H(q_k)$ and $H(d)$ for the current query $q_k$ and document $d$ through BERT:
\begin{align}
    H(q_k) &= \text{BERT}(\text{[CLS]}; q_1; \text{[SEP]}; \dots; \text{[SEP]}; q_k; \text{[SEP]});\label{eq:convdr:q} \\
    H(d) &= \text{BERT}(\text{[CLS]}; d ; \text{[SEP]}).
\end{align}
The representations of the first token [CLS] are regarded as representations of query $q_k$ and document $d$, which are denoted as $H_0(q_k)$ and $H_0(d)$, respectively. The relevance score $f(q_k, d)$ can be calculated by a simple dot product operation:
\begin{align}
    f(q_k, d) = (H_0(q_k))^T \cdot H_0(d).
\end{align}


The conversational dense retriever can be optimized to learn query and document representations with the negative log likelihood (NLL) loss:
\begin{equation}\label{eq:rank_loss}
    \mathcal{L}_{Rank}=-\log \frac{\exp \left(f\left(q_k, d^{+}\right)\right)}{\exp \left(f\left(q_k, d^{+}\right)\right)+\sum\limits_{d^{-} \in D^{-}} \exp \left(f\left(q_k, d^{-}\right)\right)},
\end{equation}
where $d^+$ and $d^-$ are relevant and irrelevant documents for $q_k$, respectively. To form the negative document set $D^-$, we retrieve negative documents ranked top by ANCE with the manually reformulated query $\tilde{q}_k$ of $q_k$. During inference, we use FAISS~\cite{johnson2019billion} to conduct efficient nearest neighbor search and find relevant documents from the pre-computed document index.


For reranking stage, we can directly concatenate all queries $\{q_i\}_{i=1}^{k}$ and document $d$ to calculate the token representations $H(q_k,d)$, which is similar to E.q.~\ref{eq:rerank:qr}:
\begin{equation}
     H(q_k,d) = \text{BERT} (\text{[CLS]};q_1;\text{[SEP]};\dots;\text{[SEP]};q_k;\text{[SEP]}; d;\text{[SEP]}), 
\end{equation}
where the representation $H_0(q_k,d)$ of the first token [CLS] is regarded as the ranking feature. Then the $H_0(q_k,d)$ is used to calculate the reranking score similar to E.q.~\ref{eq:rerank:mlp}.

\subsection{Few-Shot from Ad Hoc Dense Retriever}\label{model:kd}
\input{Figures/fig-method}
Dense retrieval usually requires large-scale relevance labels and sophisticated training strategies to guarantee its advance~\cite{xiong2020approximate, gao2020complementing, luan2020sparse}.
Nevertheless, conversational search is few-shot and lacks relevance labels for training, which derives from the complex, personalized, and tail conversational sessions.

To alleviate the data dependency, conversational retrieval can inherit the same document representations learned in ad hoc retrieval models, such as ANCE~\cite{xiong2020approximate}, which share the same information with the conversational search. Thus, we focus on understanding complex conversational queries, learning query representations, and mapping these queries in the learned document embedding space of ANCE for text retrieval. We design a teacher-student framework by training the representation of $q_k$ to mimic the representations of manually reformulated query $\tilde{q}_k$ from our teacher model ANCE.


Given the current query $q_k$, we can get its representations $H_0(q_k)$ through the query encoder from \convance{}, which is same as Eq.~\ref{eq:convdr:q}. Then we can get an approximate representation $\tilde{H}(\tilde{q}_k)$ for $q_k$'s manually reformulated query $\tilde{q}_k$ from the query encoder of the teacher model ANCE:
\begin{equation}
    \tilde{H}(\tilde{q}_k) = \text{BERT}(\text{[CLS]}; \tilde{q}_k ; \text{[SEP]}),
\end{equation}
The representation of the manually reformulated queries $\tilde{q}_k$ is [CLS]'s representation and is denoted as $\tilde{H}_0(\tilde{q}_k)$.
Then we optimize \convance{} to produce the query representation $H_0(q_k)$ of $q_k$ that is asymptotic to the representation $\tilde{H}_0(\tilde{q}_k)$ of the manually reformulated query with the knowledge distillation (KD) loss $\mathcal{L}_{\text{KD}}$:
\begin{align}\label{eq:KD_loss}
    \mathcal{L}_{\text{KD}} = \text{MSE}(H_0(q_k), \tilde{H}_0(\tilde{q}_k)),
\end{align}
where MSE denotes the Mean Square Error (MSE) loss function. In the knowledge distillation training $\mathcal{L}_{\text{KD}}$, we regard ANCE as a teacher to guide \convance{} learn tailored representations for conversational queries in the document embedding space of ANCE.

Besides, we can also incorporate the knowledge distillation loss $\mathcal{L}_{\text{KD}}$ (Eq.~\ref{eq:KD_loss}) with the general ranking loss $\mathcal{L}_{\text{Rank}}$ (Eq.~\ref{eq:rank_loss}) through multi-task training to improve few-shot ranking performance. The multi-task training loss $\mathcal{L}$ can be calculated:
\begin{align}
    \mathcal{L} = \mathcal{L}_{\text{KD}} + \mathcal{L}_{\text{Rank}}.
\end{align}

The KD training paradigm directly optimizes \convance{} by mimicking representations of manual rewritten queries, which transfers ranking knowledge from well-trained ad hoc retriever to conversational retriever through the teacher-student mechanism~\cite{hinton2015distilling,wang2020knowledge}. KD has been widely used to enable human to quickly learn complex concepts and show the effectiveness of guiding the student network learn~\cite{chung2020feature,kim2018paraphrasing,hinton2015distilling}. Benefited from teacher-student interactions, the student model can learn complex ranking patterns on few-shot scenarios~\cite{gutstein2008knowledge}, helping alleviate the data dependency of conversational retrieval. 
Moreover, these training paradigms can also be extended to BERT rerankers and conduct variant reranking models.


==> Arxiv/04_exp.tex <==
\section{Experimental Methodology}
This section describes our experimental settings, baselines, and implementation details of \convance{}.


% \subsection{Datasets}
\textbf{Datasets.} We use two conversational search benchmarks in our experiments, TREC CAsT 2019~\cite{dalton2020cast} that is few-shot, and OR-QuAC~\cite{qu2020orqa} where the search task is syntactic but include a large amount of labels.
% that consists of fully synthetic supervision. 
The data statistics of these two datasets are presented in Table~\ref{tab:dataset}.

\input{Tables/tab-dataset}

\textit{CAsT-19.} TREC Conversational Assitance Track (CAsT) 2019 dataset~\cite{dalton2020cast} consists of a series of dialogues (topics) for conversational search. There are 30 training dialogues and 50 test dialogues in CAsT-19 and each dialogue contains an average of 9 to 10 queries in natural language. Queries in a dialogue are constructed manually to mimic a "real" dialogue on a certain topic. Conversational queries have common natural language features including coreferences, abbreviations, and omissions towards mentioned concepts, making later turns depend on previous utterances. The retrieved documents are passages collected from MS MARCO and TREC Complex Answer Retrieval Paragraph Collection. Relevance judgments are provided for 20 test topics by pooling and judging submitted runs. The main evaluation metric is NDCG@3. MAP@10 and MRR are also evaluated. CAsT-19 provides manually rewritten queries that are de-contextual and independent for all test topics.

\textit{OR-QuAC.} OR-QuAC~\cite{qu2020orqa}, a large-scale synthetic conversational retrieval dataset, is built on a conversational QA dataset QuAC~\cite{choi2020quac}. The annotators to ask multi-turn questions about a given Wikipedia entity and its description, which is not the ``real'' conversation scenario. OR-QuAC extends QuAC to the open-retrieval setting by employing a document collection from the English Wikipedia dump of 10/20/2019. OR-QuAC reserves queries that have rewrites in CANARD~\cite{elgohary2019canard} and annotates passages that contain the golden answer as relevant ones for the given query. To keep the same evaluation with previous work~\cite{qu2020orqa}, we use MRR@5, Recall@5, and MAP@10 for evaluation. MRR@5 is the main evaluation metric.
\input{Tables/tab-overall-results}
% \subsection{Baselines}

\textbf{Baselines.} The baselines can be classified into two groups, published baselines, and our implemented baselines. Published baselines reformulate queries and employ a two-stage retrieval pipeline that uses a sparse/dense method for retrieval and BERT for reranking. Our implemented baselines mainly focus on the retrieval stage.


We first compare three published models for CAsT-19, \texttt{pgbert}, \texttt{h2oloo\_RUN2} and \texttt{CFDA\_CLIP\_RUN7}, which ranked top in the CAsT 2019 shared task~\cite{cast2019overview}. \texttt{pgbert}~\cite{cast2019overview} first fine-tunes GPT-2~\cite{radford2019language} on the query rewriting task using the queries from QuAC~\cite{choi2020quac} and CANARD~\cite{elgohary2019canard}. Then it uses rewritten queries to retrieve documents with Anserini~\cite{yang2017anserini} and rerank them with a BERT-based model. \texttt{h2oloo\_RUN2}~\cite{yang2019query} uses topic title for BM25 retrieval and adopts Historical Query Expansion (HQE), a heuristic method, to expand queries from conversation history for BERT reranking. \texttt{CFDA\_CLIP\_RUN7}~\cite{yang2019query} employs the same ranking pipeline as \texttt{h2oloo\_RUN2} except using doc2query~\cite{nogueira2019document} to expand MS MARCO paragraphs. We also compare \texttt{RRF (Reranking)}, which conducts reciprocal rank fusion~\cite{cormack2009reciprocal} towards ranking results provided by HQE and Neural Transfer Reformulation (NTR). NTR uses a T5~\cite{t5-model} based query rewriter to reformulate queries. For OR-QuAC, we compare its official baseline \texttt{ORConvQA}~\cite{qu2020orqa}. \texttt{ORConvQA} is an end-to-end neural QA system including a dense retriever, a reranker and a reader. The dense retriever concatenates the current and historical utterances for retrieval.

For our implemented baselines, we consider different query formats and employ BM25 or ANCE~\cite{xiong2020approximate} as our retrievers. First, we directly use the raw queries in conversations to retrieve documents and conduct two baselines, \texttt{BM25-Raw} and \texttt{ANCE-Raw}. Then we follow previous work~\cite{yu2020few} to use the pretrained generator model GPT-2 to rewrite queries and conduct two query rewriting baselines, \texttt{BM25-Query Rewriter} and \texttt{ANCE-Query Rewriter}, which are regarded as our main baselines. For CAsT-19, we follow the Yu et al.~\cite{yu2020few}'s \texttt{Rule-Based+CV} setting to first train the query rewriter on rule-based weak supervision data and then do five-fold cross-validation on the CAsT test set. For OR-QuAC, we train the query rewriter on the training set of OR-QuAC.

\textbf{Manual Reference.} The manual baselines take manually rewritten queries as input and use them for retrieval. The retrieval performance of manually rewritten queries is usually regarded as the golden standard of reformulated queries~\cite{kumar2020making} and are crucial baselines to evaluate the effectiveness of query rewriters. We employ two kinds of retrievers in our experiments, a sparse retriever BM25 that is widely used in previous work~\cite{yu2020few,kumar2020making,cast2019overview} and the state-of-the-art dense retriever ANCE~\cite{xiong2020approximate}, to conduct two baselines \texttt{BM25-Manual} and \texttt{ANCE-Manual}.


\textbf{Implementation Details.} For both \convance{} and BERT reranker, we conduct three training paradigms as shown in Section~\ref{model}, yielding three model variants, \texttt{KD} to distill ranking knowledge, \texttt{Rank} to learn ranking preference and \texttt{Multi-Task} that incorporates both ranking losses from \texttt{KD} and \texttt{Rank}. For \convance{}, we conduct three kinds of models, including \texttt{\convance{} (KD)}, \texttt{\convance{} (Rank)} and \texttt{\convance{} (Multi-Task)}. For BERT reranker, we conduct \texttt{BERT (KD)}, \texttt{BERT (Rank)} and \texttt{BERT (Multi-Task)}. To evaluate the effectiveness of training, we compare zero-shot models, \texttt{\convance{} (Zero-Shot)} and \texttt{BERT (Zero-Shot)}, in our experiments, which are trained only with the ad hoc retrieval tasks.

\textit{\convance{}.} ANCE is a state-of-the-art dense retriever and is trained on the same data sources with CAsT-19 and OR-QuAC. We borrow the checkpoints from ANCE to initialize \convance{}. For CAsT-19, we directly use the official checkpoint of the 600k-th step trained on the MS MARCO passage ranking task. For OR-QuAC, we start from the official ANCE checkpoint trained on Natural Questions~\cite{nq} and TriviaQA~\cite{triviaqa} and continuously train \convance{} on the training set of OR-QuAC with manually rewritten queries, where we use 3 GPUs, employ Adam optimizer with the learning rate of 1e-6 and set batch size to 6 during training. After initializing, we encode documents as dense representations and keep them fixed. In the training process of \convance{}, we only fine-tune its query encoder. We concatenate current and historical queries as input and truncate it with the max sequence length of 256. All variances of \convance{} are trained with 8 epochs on CAsT-19 and trained with 1 epoch on OR-QuAC. During training, we use 1 GPU, set the batch size to 4, and set the learning rate to 1e-5. For the \texttt{\convance{} (Rank)} and texttt{\convance{} (Multi-Task)}, we use the manual rewrites to retrieve documents with vanilla ANCE and sample top 9 negatives documents for each query to construct the negative document set. 

\textit{BERT Reranker.} We train BERT rerankers on MS MARCO Passage Ranking task and OR-QuAC with manually reformulated queries. Then we use different query formats to fine-tune BERT and conducts \texttt{BERT-Raw}, \texttt{BERT-Query Rewriter}, \texttt{BERT-Manual} and \texttt{BERT} with raw, query rewriter based, manually reformulated, and concatenated queries. We use 4 GPUs to train BERT with Adam optimizer, set the learning rate to 3e-6, and set the batch size to 32.

==> Arxiv/05_evaluation.tex <==
\section{Evaluation Result}
\label{result}
The experiments are conducted to study the performance of \convance{}, the effectiveness of different training strategies and the advantages of \convance{} on learning representations for conversational queries. Finally, case studies are also conducted.


\subsection{Overall Performance}\label{result:overall}
The ranking performance of \texttt{\convance{}} and baselines on CAsT-19 and OR-QuAC datasets is shown in Table~\ref{tab:result}.

For CAsT-19, the top three submitted automatic runs in the CAsT 2019 shared task, \texttt{pgbert}, \texttt{h2oloo\_RUN2} and \texttt{CFDA\_CLIP\_RUN7}, and the later model \texttt{RRF (Reranking)} are compared. These models mainly focus on expanding or reformulating the conversational queries to retrieve documents with sparse models, such as BM25, and rerank them with BERT. 
\texttt{\convance{} w/ BERT} conducts the best performance on all testing scenarios, showing its effectiveness on the few-shot conversational retrieval task. On OR-QuAC, \convance{} shows great improvement by achieving more than 100\% improvement compared with the previous state-of-the-art \texttt{ORConvQA}. Such impressive improvement further confirms the effectiveness of \convance{} and demonstrates the generalization ability of \convance{}.

\input{Tables/tab-efficiency}
Then we evaluate the ranking performance of sparse retriever and dense retriever with different query formats, \texttt{Raw}, \texttt{Query Rewriter} and \texttt{Manual}. \texttt{Raw} and \texttt{Manual} denote the queries without reformulation and with manual reformulation. \texttt{Query Rewriter} uses Yu et al.'s work~\cite{yu2020few} to reformulate queries. We first evaluate the effectiveness of different retrievers, ANCE and BM25.
In the retrieval stage, the dense retriever ANCE significantly outperforms the sparse retriever BM25 on all testing scenarios, illustrating that dense retriever achieves better ranking performance by overcoming the vocabulary mismatch problem. However, when we employ BERT to rerank selected documents from these retrievers,  ANCE-based models show distinct performance. It probably derives from that ANCE has stronger ability to choose more difficult documents~\cite{xiong2020approximate}, while the BERT reranker is not well trained to distinguish these retrieved documents in the few-shot training scenarios, such as CAsT-19.

We further evaluate the retrieval effectiveness of different query formats with various retrievers. For both \texttt{BM25} and \texttt{ANCE}, The query reformulation model \texttt{Query Rewriter}~\cite{yu2020few} significantly outperforms \texttt{RAW}, while underperforms \texttt{Manual}, demonstrating that the query rewriter has the ability to generate more informative and de-contextual queries but still has a gap with the manually reformulated queries. Different from \texttt{Raw}, \texttt{Query Rewriter} and \texttt{Manual}, \convance{} directly encodes the current query and its historical utterances without any query reformulations. \convance{} significantly outperforms \texttt{ANCE-Query Rewriter} by achieving 13.9\% and 34.8\% improvements compared with \texttt{ANCE-Query Rewriter} on CAst-19 and OR-QuAC, and achieves even better performance than \texttt{ANCE-Manual}. It demonstrates that \convance{} has the ability to summarize necessary information from historical utterances, better comprehend conversational queries and learn more tailored query representations without labored query reformulation or expansion. Moreover, when we use BERT as reranker, \texttt{\convance{} w/ BERT} also outperforms \texttt{BM25-Query Rewriter w/ BERT-Query Rewriter} with 11.6\% and 37.8\%, which illustrates that the advances of \convance{} in the retrieval stage can be extended to the whole conversational retrieval pipeline.

\subsection{Efficiency of \convance{} Retrieval}
Table~\ref{tab:efficiency} presents the efficiency of \convance{} and traditional conversational retrieval pipelines on both datasets. The speed is measured per query. The traditional \texttt{BM25-Query Rewriter} model is time-consuming, which is attributed to the inefficient self-regressed query rewriting and the slow BM25 retrieval. \convance{} provides an efficient end-to-end neural retrieval solution by directly encoding the query and performing batched nearest neighbor search on GPUs, resulting to over 40x speedup over traditional models. 

\input{Tables/tab-ablation}
\input{Tables/tab-win-tie-loss}

\subsection{Ablation Study}
This subsection explores the effectiveness of different training strategies. We evaluate the performance of \convance{} and BERT reranker trained with different training paradigms, including \texttt{Rank}, \texttt{KD} and \texttt{Multi-Task}. \texttt{Zero-Shot} that without training with conversational data is also compared in our experiments.

\textbf{\convance{} Training Paradigm Ablation:} As shown in Table~\ref{tab:ablation}, we first present the overall performance of different \convance{} variants. \convance{} focuses on learning better representations for conversational queries and shows distinct results on CAsT-19 and OR-QuAC datasets. On CAsT-19, \texttt{KD} makes a great leap compared to \texttt{Zero-Shot}, demonstrating that \texttt{KD} is effective to learn tailored representation for conversational queries and map these queries into the well-trained embedding space of ad hoc retriever ANCE in few-shot scenarios. On the contrary, the \texttt{Rank} and \texttt{Multi-Task} models yield poor ranking results, indicating severe overfitting when supervised with few ranking labels. When trained with a larger dataset OR-QuAC, \texttt{Rank} benefits from the end-to-end training with massive relevance labels, showing more effectiveness compared to \texttt{KD}. \texttt{Multi-Task} brings further improvements to \texttt{Rank} with the help of additional knowledge distillation training paradigm (\texttt{KD}), demonstrating that \texttt{KD} still helps to learn better query representations trained with ranking preference signals when a large amount of training data is available.

\textbf{BERT Ranker Training Paradigm Ablation:} Then the variant of \convance{} with the best performance is chosen as the first stage retriever to evaluate the performance of BERT rerankers optimized with different training strategies. \texttt{Multi-Task} usually achieves the best performance among all training strategies but show little improvement compared with \texttt{Zero-Shot}. BERT reranker shows its ability to establish effective interactions between queries and documents to estimate their relevance, which thrives from training with ad hoc retrieval tasks. Besides, \texttt{KD} conducts more stable performance on the few-shot scenario, while \texttt{Rank} performs better when trained with a larger dataset, which are consistent with the observations of \convance{}.


\textbf{Win/Tie/Loss Study:} We further verify the effectiveness of \convance{} optimized with different training paradigms through a Win/Tie/Loss study by comparing with two ANCE baselines with \texttt{ANCE-Query Rewriter} and \texttt{ANCE-Manual}, as shown in Table~\ref{tab:wtl}. Both \texttt{ANCE-Query Rewriter} and \texttt{ANCE-Manual} use vanilla ANCE as encoder and feed reformulated queries from query rewriter and manual annotations to get query representations. On both datasets, \texttt{KD} shows higher tie rates compared with \texttt{ANCE-Manual}, showing its effectiveness on mimicking manual representations. Furthermore, \texttt{KD} conducts more Win cases than Loss cases compared with both automatically reformulated queries and manually rewritten queries, which shows that teaching \convance{} learn  asymptotic representations of manual rewrites can learn beyond what it is taught and break the performance ceiling of query reformulation or expansion systems. \texttt{Rank} can improve the query representation ability of \convance{} only trained with enough relevance signals, which is consistent with previous findings. Integrated with \texttt{KD}, \texttt{Multi-Task} conducts significant less Loss cases on OR-QuAC, leading to further improvement. These training paradigms guide \convance{} learn query representations from different training directions and guarantee the effectiveness of \convance{} on different scenarios. 

\input{Figures/fig-rep-q}
\input{Figures/fig-rep-qd}
\input{Figures/fig-round}
\input{Figures/fig-overlap}
\subsection{Query Representations of \convance{}}
In this part, we study the effectiveness of \convance{} by exploring the distribution of various query representations in the embedding space. Several baselines are employed to provide query representations with different query formats:  \texttt{ANCE-Query Rewriter}, \texttt{ANCE-Manual} and \texttt{\convance{} (Zero-Shot)}.

\textbf{Query Representation Distributions:} We first investigate the distribution of query representations from different models, as shown in Figure~\ref{fig:query-reps}. We show the average distance between different query representations in Figure~\ref{fig:query-sim}. The representation of \texttt{\convance{} (Zero-Shot)} shows low similarity with others, especially for the current raw queries, indicating that \texttt{\convance{} (Zero-Shot)} fails to distinguish the more important conversational round in the historical utterances to learn a tailored representation for the current query. With the help of a query rewriter, \texttt{\convance{} (Query Rewriter)} obtains a highly similar representation to \texttt{ANCE-Manual} while keeping a fair similarity with \texttt{ANCE-Raw}, showing the success of query rewriter in transforming the raw queries into the manual-like form. \texttt{\convance{} (KD)} is also closer to \texttt{ANCE-Manual}, which confirms its effectiveness on learning necessary information from historical utterances. However, \texttt{\convance{} (KD)} also shows almost same similarity scores with \texttt{\convance{} (Query Rewriter)} and \texttt{ANCE-Manual}, as well as conducts more closer representations to \texttt{ANCE-Raw}, demonstrating \texttt{\convance{} (KD)} considers more about the raw inputs instead of overfitting to the manual queries.


Then we further choose one case to analyze the effectiveness of \texttt{\convance{} (KD)} through visualizing the representation distribution of different queries, as shown in Figure~\ref{fig:query-tsne}. \texttt{\convance{} (Zero-Shot)} is the initial state of \texttt{\convance{} (KD)} and always distracted by the utterances from previous rounds. After training, the representation of \texttt{\convance{} (KD)} is more closer to \texttt{ANCE-Manual} and the representation of the current query (Q6) compared with the representation of \texttt{\convance{} (Zero-Shot)}. It demonstrates that \texttt{\convance{} (KD)} has the ability to focus more on the current query and learns a more meaningful representation for the current query. However, \texttt{\convance{} (KD)} shows not identical performance with \texttt{ANCE-Manual}. It is pulled more closer to the historical query representations than \texttt{ANCE-Manual}. Such difference indicates that, by embedding the whole conversation history, \texttt{\convance{} (KD)} also learns some valuable information from previous conversational rounds that does not appear in the manual rewrites.



\textbf{Query Representations in Document Embedding Space:} Finally, as shown in Figure~\ref{fig:qd}, we take a deep look at the query representation distribution in the document embedding space. We statistically calculate the average similarity scores between queries and their nearest positive document in Figure~\ref{fig:qd-sim}. \texttt{ANCE-Manual} encodes manually annotated queries and is usually regarded as the upper bound of query reformulation based models. We find that \texttt{ANCE-Query Rewriter} has the lowest similarity score among all models and shows a larger margin compared with \texttt{ANCE-Manual}, which derives from the underperforming query rewriter. Compared with \texttt{ANCE-Manual}, \texttt{\convance{} (KD)} shows a higher similarity score, verifying the effectiveness of \texttt{\convance{} (KD)} on learning query representations that are closer to relevant documents. Then we also conduct a case to intuitively show the representation distribution of queries and documents in Figure~\ref{fig:qd-tsne}. Overall, \texttt{\convance{} (Zero-Shot)} is distributed closer to irrelevant documents, while others are located closer to relevant documents, which illustrates \texttt{ANCE-Manual}, \texttt{ANCE-Query Rewriter} and \texttt{\convance{} (KD)} can learn a better representations for retrieval even with different query formats. Compared with \texttt{ANCE-Manual} and \texttt{ANCE-Query Rewriter}, \texttt{\convance{} (KD)} occupies a more central position among all relevant documents and conducts a more closer representation to relevant documents on average, which helps to assign more relevant documents with top ranks and achieves better ranking performance for conversational retrieval.


\input{Tables/tab-case-new}
\subsection{\convance{} with Muti-turn Conversation}
In this subsection, we further conduct experiments to study the effectiveness of \convance{} on learning query representations from multi-turn conversations, as shown in Figure~\ref{fig:round} and ~\ref{fig:overlap}.

For the first experiment, we evaluate the ranking performance of \convance{} at different conversational turns in Figure~\ref{fig:per-turn}. With the conversation goes on, \texttt{ANCE-Raw} usually conducts poor retrieval performance and achieves only about 0.2 NDCG@3 score. \texttt{ANCE-Query Rewriter} shows its effectiveness and significant improves ranking performance by reformulating the conversational queries to alleviate the context dependency. Nevertheless, when the conversational turn is larger than 8, \texttt{ANCE-Query Rewriter} and \texttt{\convance{} (KD)} show distinct performance. The performance of \texttt{ANCE-Query Rewriter} dramatically decreases, because comprehending queries with long conversational history is much harder than shallow conversations. On the contrary, \texttt{\convance{} (KD)} maintains a more stable performance compared with \texttt{ANCE-Query Rewriter}, which shows its robust and strong ability to model query representations with deeper conversations. Besides, compared with \texttt{ANCE-Manual}, \texttt{\convance{} (KD)} usually performs better, while \texttt{ANCE-Query Rewriter} performs worse in the conversational retrieval scenarios of different depths, demonstrating that \texttt{\convance{} (KD)} can better understand conversational queries and conduct more tailored query representations than query rewriters. To further investigate how well \convance{} maintains user's information need as the conversation proceeds, we present the similarity score between the current turn and its previous turn in Figure~\ref{fig:turn-sim}. We find that \texttt{\convance{} (KD)} keeps the highest similarity with previous turns, indicating that \texttt{\convance{} (KD)} is able to grasp the conversation ``topic'' and coherently understand query intent based on the conversation history.

Then we evaluate whether \convance{} has the ability to attend more important utterances in conversations for learn query representations. We randomly mask one piece of utterances in a history and calculate the similarity score (dot product score) between representations before and after masking. Then we plot the data point distribution to study how the similarity score change with the ``importance'' of masked utterances that is evaluated by term overlap between the masked utterance and the manually rewrite of the current query. The data distributions of \texttt{\convance{} (Zero-Shot)}, \texttt{ANCE-Query Rewriter} and \texttt{\convance{} (KD)} are shown in Figure~\ref{fig:overlap-zs}, Figure~\ref{fig:overlap-qr}, and Figure~\ref{fig:overlap-kd}, respectively. For \texttt{\convance{} (Zero-Shot)}, the data points are most concentrated into the interval of similarity score from 710 to 720. Such insensitive changes of similarity scores indicate the degenerate representation ability for ad hoc retriever in the conversational retrieval scenario. Compared with \texttt{\convance{} (Zero-Shot)}, \texttt{ANCE-Query Rewriter} conducts a more scattered data points distribution, which is that similarity scores of these data points are more significantly changed when the utterances of higher quality are masked. \texttt{\convance{} (KD)} is more like a trade-off distribution of \texttt{\convance{} (Zero-Shot)} and \texttt{ANCE-Query Rewriter}. The masked utterance with different quality also has discriminate influence in the query representation of \texttt{\convance{} (KD)}, while the changes are not such dramatic with the changes of \texttt{ANCE-Query Rewriter}, which illustrates that \texttt{\convance{} (KD)} directly encodes the current and historical utterances in a conversation to fully understand queries and avoid directly overfitting to manually reformulated queries. Data points of \texttt{\convance{} (Multi-Task)} are nearly uniform on overlap ratio, demonstrating that it fails to distinguish important terms from unimportant ones.


\subsection{Case Study}
In the rest of this section, we provide three cases sampled from CAsT-19 to further evaluate the effectiveness of \convance{}, as shown in Table~\ref{tab:case}.

In the first case, we evaluate the retrieval performance of \texttt{\convance{} (KD)} compared with \texttt{ANCE-Manual}. The concept ``ACL'' of current query is an ambiguous concept that may be an abbreviation for ``Access Control List'' or ``Anterior Cruciate Ligament''. It is apparent that in this conversation ``ACL'' means ``Anterior Cruciate Ligament'' because the historical utterances have mentioned some related words to help comprehend this concept, such as ``sports'' and ``injuries''. Human annotators only focus on reformulating an de-contextual queries instead of completing necessary semantic information for queries. Thus, the manually reformulated query keeps same with the raw query, which is unclear and misleads retriever to retrieve documents about different semantics of ``ACL''. On the contrary, \texttt{\convance{} (KD)} shares some attentions to utterances from previous rounds and conducts more informative representations for retrieval.

For another two cases, we compare the retrieval performance of \texttt{\convance{} (KD)} and our main baseline \texttt{ANCE-Query Rewriter}. In the second case, the query rewriter provides a wrong reformulation result. According to the 5-th and 6-th rounds, the current query talks about ``Milgram experiment'' instead of ``Stanford Experimen''. Such defective query rewrite leads the search results stray off the discussion topic and harm user experience. \texttt{\convance{} (KD)} directly encodes all utterances and avoids involving extra errors from explicitly reformulated queries. Moreover, \texttt{\convance{} (KD)} focuses more on the utterance about ``Milgram experiment'' than the utterance about ``Stanford Experimen'', which helps to learn more accurate query representation for retrieval. In the third case, the complex conversation becomes an obstacle for understanding the current query and pushes the query rewriter maintain the same utterance with the raw query. Different from the shallow understanding of query rewriter, \texttt{\convance{} (KD)} shows more meaningful representations by considering the historical utterances talked about ``Darwin’s theory'', ``reproduction'' and ``biology'', which helps better comprehend the current query.

==> Tables/tab-case.tex <==
\begin{table*}
    \caption{Case study. Snippets are manually extracted. The documents in the first disagreed ranking position are shown, where on all examples \convance{} won.}
    \label{tab:case} 
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{l|p{0.4\linewidth} | p{0.4\linewidth}} 
    \hline
                    & \textbf{\convance{} (KD)}         & \textbf{ANCE-Manual}      \\
    \hline
    Conversation    & \multicolumn{2}{l}{\begin{tabular}{@{}l@{}}Which weekend sports have the most injuries? [-1.07]\\ 
                      What are the most common types of injuries? [-0.53]\\
                      \textbf{What is the ACL?} [-10.67] \end{tabular}}       \\
    \hline
    Rewrite         & n.a.                              & What is the ACL?          \\
    \hline
    Doc Snippet     & An ACL injury is the tearing of the anterior cruciate (KROO-she-ate) ligament (ACL) ... one of the major ligaments in your knee ...
                                                        & ACL. Short for Access Control List, an ACL is a list containing one or more ACE which are used by an operating system or ...  \\
    %\hline
   % Ranking position& 2                                 & 2 \\
    %\hline
    %Label           & 4                                 & 0 \\
    %\hline
   % NDCG@3          & 0.691                             & 0.469 \\
    \hline
    Conversation    & \multicolumn{2}{l}{\begin{tabular}{@{}l@{}} What is worth seeing in Washington D.C.? [-0.19] \\
                     Which Smithsonian museums are the most popular? [-0.09] \\
                     Why is the National Air and Space Museum important? [-0.07] \\
                     Is the Spy Museum free? [-0.08] \\
                     What is there to do in DC after the museums close? [-0.19] \\
                     What is the best time to visit the reflecting pools? [-0.09] \\
                     Are there any famous foods? [-0.00] \\
                     \textbf{What is a DC half smoke? } [-15.55] \end{tabular}}       \\
    \hline
    Rewrite         & n.a.                              & What is a DC half smoke?          \\
    \hline
    Doc Snippet     & In Washington, D.C. the half-smoke is similar to a hot dog, but usually larger, spicier, and with more coarsely-ground meat, ...
                                                        & half and half. A cheap brand of all-purpose smoking tobacco - one of the earliest packaged, branded pipe tobaccos in the U.S. ...  \\
    %\hline
    %Ranking position& 3                                 & 3 \\
    %\hline
    %Label           & 4                                 & 0 \\
    %\hline
    %NDCG@3          & 1.0                               & 0.765 \\
    %\hline
    \hline
                    & \textbf{\convance{} (KD)}         & \textbf{ANCE-QR}      \\
    \hline
    Conversation    & \multicolumn{2}{l}{\begin{tabular}{@{}l@{}}What was the Stanford Experiment? [-1.51] \\
                     What did it show? [-0.10] \\
                     Tell me about the author of the experiment. [-0.22] \\
                     Was it ethical? [-0.19] \\
                     What are other similar experiments? [-0.16] \\
                     What happened in the Milgram experiment? [-3.92] \\
                     \textbf{Why was it important?} [-5.79] \end{tabular}}   \\
    \hline
    Rewrite         & n.a.                              & Why was the Stanford Experiment important? \\
    \hline
    Doc Snippet     & In 1961, in response to the Nuremberg Trials, the Yale psychologist Stanley Milgram performed his \"Obedience to Authority Study\", also known as the Milgram Experiment, in order to determine ...
                                                        & Forty years ago today, the Stanford Prison Experiment began ... arguably history ... most notorious and controversial psychology experiment, which gleaned powerful and unsettling insights into human nature. \\
    %\hline
    %Ranking position& 1                                 & 1 \\
    %\hline
    %Label           & 3                                 & 0 \\
    %\hline
    %NDCG@3          & 0.694                             & 0.0 \\
    \hline
    Conversation    & \multicolumn{2}{l}{\begin{tabular}{@{}l@{}} What is Darwin’s theory in a nutshell? [-0.77] \\
                     How was it developed? [-0.19] \\
                     How do sexual and asexual reproduction affect it? [-0.10] \\
                     How can fossils be used to understand it? [-0.01] \\
                     What is modern evidence for it? [-0.12] \\
                     What is the impact on modern biology? [-0.18] \\
                     Compare and contrast microevolution and macroevolution. [-0.37] \\
                     \textbf{What is the relationship to speciation? } [-7.05] \end{tabular}}      \\
    \hline
    Rewrite         & n.a.                              & What is the relationship to speciation? \\
    \hline
    Doc Snippet     & Speciation is the evolutionary process by which reproductively isolated biological populations evolve to become distinct species. ... Charles Darwin was the first to describe the role of natural selection in speciation in his 1859 book The Origin of Species ...
                                                        & Speciation is defined by the International Union of Pure and Applied Chemistry (IUPAC) as the distribution of an element amongst defined chemical species in a system. ... \\
    %\hline
    %Ranking position& 1                                 & 1 \\
    %\hline
    %Label           & 4                                 & 0 \\
    %\hline
    %NDCG@3          & 0.691                             & 0.0 \\
    \hline
    \end{tabular}
    }
\end{table*}

==> Tables/tab-conversation-example.tex <==
\begin{table}
  \caption{A Conversational Search Example in TREC CAsT 2019 \cx{make a figure that illustrate conv-ance in the representation space about modeling the conversational rounds}}
  \label{tab:example}
  \resizebox{0.48\textwidth}{!}{
  \begin{tabular}{cl}
    \hline
    \hline
    \multicolumn{2}{l}{\textbf{Description}:}                                           \\
    \multicolumn{2}{l}{The Bronze Age collapse and the transition into a dark age.}     \\
    \hline
    \textbf{Turn}   & \textbf{Conversational Queries}                                   \\
    \hline
    $Q_1$           & Tell me about the Bronze Age collapse.                            \\
    $Q_2$           & What is the evidence for it?                                      \\
    $Q_3$           & What are some of the possible causes?                             \\ 
    \hline
    \multicolumn{2}{l}{\textbf{Manual Query Rewrites}}                                  \\ 
    \hline
    $Q^*_2$         & What is the evidence for \textbf{the Bronze Age collapse}?        \\
    $Q^*_3$         & What are some of the possible causes \textbf{of the Bronze Age collapse}?      \\
    \hline
    \hline
  \end{tabular}}
\end{table}

==> Tables/tab-overall-results.tex <==
\begin{table*}
    \caption{Overall results on CAsT-19 and OR-QuAC. Percentages indicate relative performance over \texttt{BM25-Query Rewriter} (QR) or \texttt{BM25-QR w/ BERT-Query Rewriter} on the main evaluation metrics. Superscripts $\dagger$, $\ddagger$, $\mathsection$, and $\mathparagraph$ indicate statistically significant improvements over \texttt{BM25-Raw}$\text{}^{\dagger}$, \texttt{ANCE-Raw}$\text{}^{\ddagger}$, \texttt{BM25-Query Rewriter}$\text{}^{\mathsection}$, and \texttt{ANCE-Query Rewriter}$\text{}^{\mathparagraph}$ or their corresponding reranking results. 
    Unavailable and inapplicable results are marked by  ``n.a.'' and ``--''.
    % denote unavailable and inapplicable results.
    Best results in each group are marked \textbf{Bold}.
    }
    \small
    \label{tab:result}

    % \begin{tabular}{l | p{1.2cm}<{\centering} p{1.2cm}<{\centering} p{1.2cm}<{\centering} p{1.0cm}<{\raggedleft}| p{1.2cm}<{\centering} p{1.2cm}<{\centering} p{1.2cm}<{\centering} p{1.0cm}<{\raggedleft}} 
    \resizebox{0.99\linewidth}{!}{
     \begin{tabular}{l | lllr|lllr} 
    \hline
    \multirow{2}{*}{\textbf{Method}}     & \multicolumn{4}{c|}{\textbf{CAsT-19}}                         & \multicolumn{4}{c}{\textbf{OR-QuAC}}                \\ \cline{2-9}
                                         &\textbf{MAP@10}&\textbf{MRR}   &{\textbf{NDCG@3}} & \textbf{Rel. Gain}
                                         &\textbf{MAP@10}&\textbf{R@5}&{\textbf{MRR@5}} 
                                         &  \textbf{Rel. Gain}
                                         \\ 
    \hline
    \multicolumn{9}{l}{\textbf{Public Baselines}} \\ \hline
     \texttt{pgbert} (from~\cite{cast2019overview})& n.a.          & 0.665         & 0.413         & --           & --           & --            & --           & --\\
     \texttt{h2oloo\_RUN2} (from~\cite{cast2019overview})&n.a.& 0.714         & 0.434         & --           & --           & --            & --           & --\\
     \texttt{CFDA\_CLIP\_RUN7} (from~\cite{cast2019overview})& n.a.  & \textbf{0.715}         & 0.436         & --           & --           & --            & --           & --\\
     \texttt{RRF (Reranking)} (from~\cite{lin2020query}) & n.a.   & n.a.          & \textbf{0.536}     & --           & --           & --            & --           & --\\
     \texttt{Auto-Rewriter} (from~\cite{yu2020few}) & n.a.   & n.a.          & 0.492          & --           & --           & --            & --           & --\\
     \texttt{ORConvQA reranker} (from~\cite{qu2020orqa}) & --            & --            & --            & --           & n.a.         & \textbf{0.314}         & \textbf{0.313}        & --\\
    \hline
    \multicolumn{9}{l}{\textbf{First Stage Retrieval Only}} \\ \hline
     \texttt{BM25-Raw}                 & 0.031         & 0.321         & 0.134         & -51.6\%      & 0.050        & 0.075         & 0.049        & -75.8\%\\
     \texttt{ANCE-Raw}                 & 0.045$\text{}^{\dagger}$ & 0.418$\text{}^{\dagger}$& 0.246$\text{}^{\dagger}$ & -11.0\%      & 0.114$\text{}^{\dagger}$ & 0.149$\text{}^{\dagger}$& 0.113$\text{}^{\dagger}$   & -43.8\%\\
     \texttt{BM25-Query Rewriter}      & 0.071$\text{}^{\dagger \dagger}$& 0.577$\text{}^{\dagger \dagger}$& 0.276$\text{}^{\dagger}$& +0.0\%       & 0.200$\text{}^{\dagger \dagger}$& 0.302$\text{}^{\dagger \dagger}$ & 0.202$\text{}^{\dagger \dagger}$ & +0.0\%\\
     \texttt{ANCE-Query Rewriter}      & 0.088$\text{}^{\dagger \dagger \mathsection}$& 0.661$\text{}^{\dagger \dagger \mathsection}$& 0.407$\text{}^{\dagger \dagger \mathsection}$& +47.6\%& 0.451$\text{}^{\dagger \dagger \mathsection}$& 0.584$\text{}^{\dagger \dagger \mathsection}$& 0.457$\text{}^{\dagger \dagger \mathsection}$& +126.4\%\\
     \convance{}                         & \textbf{0.094}$\text{}^{\dagger \dagger \mathsection}$& \textbf{0.735}$\text{}^{\dagger \dagger \mathsection \mathparagraph}$& \textbf{0.464}$\text{}^{\dagger \dagger \mathsection \mathparagraph}$& +68.1\%      &\textbf{0.607}$\text{}^{\dagger \dagger \mathsection \mathparagraph}$& \textbf{0.750}$\text{}^{\dagger \dagger \mathsection \mathparagraph}$&\textbf{0.616}$\text{}^{\dagger \dagger \mathsection \mathparagraph}$& +205.5\%\\
    \hline
    \multicolumn{9}{l}{\textbf{With BERT Reranker}} \\ \hline
     \texttt{BM25-Raw w/ BERT-Raw}   & 0.057         & 0.500$\text{}^{\dagger}$& 0.304$\text{}^{\dagger}$& -38.2\%      & 0.154        & 0.171         & 0.157        & -71.7\%\\
     \texttt{ANCE-Raw w/ BERT-Raw}   & 0.054         & 0.447         & 0.273         & -44.5\%      & 0.174$\text{}^{\dagger}$& 0.207$\text{}^{\dagger}$& 0.177$\text{}^{\dagger}$ & -68.1\%\\
     \texttt{BM25-QR w/ BERT-Query Rewriter}& 0.113$\text{}^{\dagger \dagger}$& 0.775$\text{}^{\dagger \dagger}$& 0.492$\text{}^{\dagger \dagger}$& +0.0\%      & 0.537$\text{}^{\dagger \dagger}$& 0.615$\text{}^{\dagger \dagger}$& 0.554$\text{}^{\dagger \dagger}$ & +0.0\%\\
     \texttt{ANCE-QR w/ BERT-Query Rewriter}& 0.117$\text{}^{\dagger \dagger}$& 0.743$\text{}^{\dagger \dagger}$& 0.479$\text{}^{\dagger \dagger}$& -2.8\%       & 0.604$\text{}^{\dagger \dagger \mathsection}$& 0.710$\text{}^{\dagger \dagger \mathsection}$& 0.615$\text{}^{\dagger \dagger \mathsection}$ & +11.1\%\\
     \texttt{\convance{} w/ BERT}& \textbf{0.130}$\text{}^{\dagger \dagger \mathsection \mathparagraph}$& \textbf{0.807}$\text{}^{\dagger \dagger \mathparagraph}$& \textbf{0.546}$\text{}^{\dagger \dagger \mathsection \mathparagraph}$& +11.0\%      &\textbf{0.758}$\text{}^{\dagger \dagger \mathsection \mathparagraph}$& \textbf{0.850}$\text{}^{\dagger \dagger \mathsection \mathparagraph}$&\textbf{0.773}$\text{}^{\dagger \dagger \mathsection \mathparagraph}$& +39.5\%\\
    \hline
    \multicolumn{9}{l}{\textbf{Manual for Reference}} \\
    \hline
     \texttt{BM25-Manual}            & 0.096         & 0.667         & 0.345         & --           & 0.316        & 0.430         & 0.330        & --\\
     \texttt{ANCE-Manual}            & 0.101         & 0.740         & 0.459         & --           & 0.507        & 0.642         & 0.515        & --\\
     \texttt{BM25-Manual w/ BERT-Manual}& 0.133         & 0.838         & 0.544         & --           & 0.645        & 0.719         & 0.665        & --\\
     \texttt{ANCE-Manual w/ BERT-Manual}& \textbf{0.137}& \textbf{0.835}& \textbf{0.563}& --           &\textbf{0.683}& \textbf{0.778}&\textbf{0.698}& --\\
    \hline
    \end{tabular}}

\end{table*}

==> Tables/tab-win-tie-loss.tex <==
\begin{table}
    \caption{Win/Tie/Loss results (\%) compared with \texttt{ANCE-QR} and \texttt{ANCE-Manual}. Per query performance is measured with main evaluation metric (NDCG@3 for CAsT-19 and MRR@5 for OR-QuAC) and is rounded to three decimal places for comparison. }
    \label{tab:wtl}
        \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{l|rrr|rrr}
        \hline
        \multirow{2}{*}{\textbf{Method}}   & \multicolumn{3}{c|}{\textbf{ANCE-QR}}    & \multicolumn{3}{c}{\textbf{ANCE-Manual}}   \\
        \cline{2-7}
                                  & \textbf{Win}      & \textbf{Tie}      & \textbf{Loss}     & \textbf{Win}     & \textbf{Tie}     & \textbf{Loss}    \\
        \hline
        \multicolumn{7}{l}{\textbf{CAsT-19}} \\
        \hline
        \texttt{\convance{} (Zero-Shot)}   & 13       & 37       & 50       & 13      & 30      & 57      \\
        \texttt{\convance{} (Rank)}        & 4        & 25       & 71       & 3       & 19      & 78      \\
        \texttt{\convance{} (KD)}          & \textbf{42}       & 38       & 21       & \textbf{38}      & 39      & 24      \\
        \texttt{\convance{} (Multi-Task)}  & 14       & 25       & 61       & 12      & 19      & 69      \\
        \hline
        \multicolumn{7}{l}{\textbf{OR-QuAC}} \\
        \hline
        \texttt{\convance{} (Zero-Shot)}   & 24       & 67       & 8        & 24      & 61      & 16      \\
        \texttt{\convance{} (Rank)}        & 30       & 58       & 12       & 29      & 52      & 19    \\
        \texttt{\convance{} (KD)}          & 19       & 72       & 10       & 19      & 63      & 18      \\
        \texttt{\convance{} (Multi-Task)}  & \textbf{31}       & 62       & 7        & \textbf{30}      & 56      & 14      \\
        \hline
    \end{tabular}}
\end{table}
